An Automated Vulnerability Detection Framework for Smart Contracts

With the increase of the adoption of blockchain technology in providing decentralized solutions to various problems, smart contracts have become more popular to the point that billions of US Dollars are currently exchanged every day through such technology. Meanwhile, various vulnerabilities in smart contracts have been exploited by attackers to steal cryptocurrencies worth millions of dollars. The automatic detection of smart contract vulnerabilities therefore is an essential research problem. Existing solutions to this problem particularly rely on human experts to define features or different rules to detect vulnerabilities. However, this often causes many vulnerabilities to be ignored, and they are inefficient in detecting new vulnerabilities. In this study, to overcome such challenges, we propose a framework to automatically detect vulnerabilities in smart contracts on the blockchain. More specifically, first, we utilize novel feature vector generation techniques from bytecode of smart contract since the source code of smart contracts are rarely available in public. Next, the collected vectors are fed into our novel metric learning-based deep neural network(DNN) to get the detection result. We conduct comprehensive experiments on large-scale benchmarks, and the quantitative results demonstrate the effectiveness and efficiency of our approach.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/Benchmark.tex <==

We collected our corpus by retrieving bytecode for every contract deployed as of May 2019. Then, we removed the duplicated contracts. In total there are only 205,848 unique bytecodes. 
Ethereum contracts vary from simple to more complex. The number of the instructions in Ethereum contracts varies from 8 to 13,050 with average 1,545.27 and median 1,213. The number of distinct instructions in the contracts. This number varies from 7 to 57. 
In this project, we use EVM bytecode instead of smart contract source codes since most of the smart contracts’ source codes are not publicly available on public repositories. 

Due to the lack of labeled data, we run Oyente on all contracts to label them by different vulnerabilities including ordering, timestamp, mishandle exception, and reentrancy or benign. Then, we discard the contracts that Oyente could not complete the process in 60 seconds. At the end of this process, there are only 176,968 unique bytecodes. This data is our gold standard for our further process. Figure \ref{fig:pie_chart} shows the percentage of benign and vulnerabilities in smart contracts detected by Oyente. 88\% of smart contracts are benign. 6\% of smart contracts suffer from Ordering attacks.  
Besides, some of the smart contracts suffer from more than one vulnerability.  It is shown in Figure \ref{fig:multi_vul}.
 

\begin{figure}
    \centering
    \caption{Percentage of benign and vulnerabilities in the benchmark}
    \label{fig:pie_chart}
    \begin{tikzpicture}
    \pie [rotate = 180, radius = 2.0] {3/Timestamp, 1/Reentrancy, 88/Benign, 6/Ordering, 2/Mishandle exception}
    \end{tikzpicture}
\end{figure}

\begin{figure}
    \centering
    \caption{Number of smart contracts in Benchmark with one or more vulnerability}
    \label{fig:multi_vul}
     \begin{tikzpicture}[scale =0.8, transform shape]
        \begin{axis}[
        x tick label style={
		/pgf/number format/1000 sep=},
        ybar,
        enlarge y limits={0.25,upper},
        enlarge x limits=0.25,
        bar width=20pt,
        %enlargelimits=0.1,
        legend style={at={(0.5,-0.15)},
        anchor=north,legend columns=-10},
        ylabel={\#Smart contract},
        symbolic x coords={1 Vulnerability, 2 Vulnerabilities, 3 Vulnerabilities, 4 Vulnerabilities},
        xtick=data,
        nodes near coords,
        nodes near coords align={vertical},
        tick label style={rotate=45}
        ]
    
    \addplot[ybar,fill=blue] coordinates {
        (1 Vulnerability,  18437)
        (2 Vulnerabilities,  6050)
        (3 Vulnerabilities,   368)
        (4 Vulnerabilities, 17)
    };
    \end{axis}
    \end{tikzpicture}
\end{figure}



==> sections/Vulnerability.tex <==
\paragraph{Reentrancy} 
Reentrancy is a well-known vulnerability with a recent TheDAO\footnote{https://etherscan.io/address/0xbb9bc244d798123fde783fcc1c72d3bb8c189413\#code} hack. In Sept of 2016, hackers stole over 3,600,000 Ether, or 60 million US Dollars at the time by exploiting a Reentrancy vulnerability in contract code from the company TheDAO. 
Since then, developers have changed codes to limit the function being accessed from malicious code. However, still, huge numbers of old contracts are vulnerable to the Reentrancy approach.

The Reentrancy vulnerability starts from a function named \textit{fall-back} function. Every contract can only have one fall-back function. The fall-back function has no arguments and no return values. 
This function will be called in two ways: First, when a contract receives a function call but no functions match; Second, when a contract receives Ethers. In Ethereum, when a contract calls another, the current execution waits for the call to finish. This can lead to an issue when the callee makes use of the intermediate state the caller is in. In other words, a malicious contract will write an external function call in its fall-back function. 

\paragraph{Time Dependency}
Many applications in Ethereum require to obtain the timestamp to decide what operations to do. Block timestamp is typically used in two situations: as a deterministic random seed. and as a global timestamp in a distributed network, such as \cite{Castle, GovernMental}. TheRun contract is an example of the former situation. TheRun contract uses the current timestamp in order to generate random numbers and award a jackpot based on the result.
The timestamp of the contract is dependent on block timestamp, and the block timestamp must be agreed by block miners. Due to the synchronization, all contracts in the same block share the same timestamp. When miner gets a new block, it has the ability to adjust the born time of the new block. This could be 900 seconds in early Solidity versions. Although it is changed to several seconds now, it still has timestamp vulnerability.

\paragraph{Mishandled Exceptions}
There are some ways for a contract to call another, including sending instructions or 
call a contract's function directly (e.g. ContractA.FunctionB()). 
Meanwhile, and exception can be raised in callee contracts because of not enough gas, exceeding call stack limit, division by zero, array index out of bound and so on). If the exception happens, the callee contract terminates, reverts its state and returns false. 27.9\% of the contracts do not check the return values after calling other contracts via send \cite{luu2016making}. A malicious caller contract can cause the send to fail deliberately, regardless of what the callee does.
Sometimes the attacker does not receive any direct benefit other than causing other users to lose their entitlement. But, in some other examples, the attacker can get the direct benefit \cite{GovernMental, Runsmart}. These contracts pay investors interest for their investments from the subsequent investments by others. An attacker can first invest his money. Then, he can cause failure in the previous investors, so he can receive his interest earlier! 

\paragraph{ Transaction-Ordering Dependence}
Since a transaction is in the mempool for a short while, one can know what actions will occur before it is included in a block. In the Ethereum Blockchain network, only miners can decide the order of transactions in a block. Therefore, the final state of a contract depends on the miner's decision about ordering the transactions.

In this situation, the miners can cause malicious behavior. For example, a smart contract offering a prize for providing the right solution to some problem. The contract owner can modify the prize as long as it has not been awarded, and users can submit their solutions to the problem to won the prize. On the other hand, the owner can track all submissions and manage the ordering of transactions. Let's consider the scenario when there is an unprocessed user transaction with a valid submission, the miner has the ability to check it out and then submit his own transaction thus reducing the value of the prize to zero. In such a case, the owner submission will be invoked first. And, the other user not only will not win the prize, but he has also submitted the solution for free! 


\paragraph{Critical Instruction Vulnerabilities}
EVM bytecode consists of instructions that allow external smart contracts to call other smart contract code. These instructions include the CALL, CALLCODE and DELEGATECALL instruction as shown in \autoref{fig:smartcall}. The CALL instruction allows a caller smart contract to call a target smart contract which can modify the storage or variables in the target contract. CALLCODE and DELEGATECALL allow a caller smart contract to call a target smart contract and modify the variable and storage in the caller's context. 
With these capabilities, attackers can inject code that can modify a smart contract's balance, change ownership or even self destruct a smart contract and withdraw all the tokens in the contract.

\paragraph{Smart Contract Owner Hijack} 
Each smart contract has an owner when deployed. For example, \autoref{lst:paritybug} shows a code snippet for setting up a smart contract wallet for the Parity Ethereum Wallet from its GitHub repository. The \textit{initWallet} method is used to set the owner of the wallet. The \textit{initWallet} method should only be executed once in the lifetime of the smart contract. After initiating a smart contract, allowing changes to the ownership of a contract through a call to \textit{initWallet} can allow an arbitrary user to use methods such as delegate call to change the ownership of the contract. With the delegatecall instruction, an attacker can pass a malicious payload to execute in the attacker's context. In this case, the attacker modified the owners of the smart contract by executing the \textit{initWallet} method. After changing the owner of the wallet contract, the attacker is able to kill the contract which results in all the funds in the wallet being withdrawn to the attacker.
High-value attacks on the Parity Multisig smart contract~\cite{codewallet}~\cite{paritybug}~\cite{tether} were completed using this vulnerability to hijack the ownership of the smart contract.

\paragraph{Arithmetic Vulnerabilities}
\label{arithvul}
Arithmetic vulnerabilities such as integer overflow and underflow can occur during EVM code execution leading to loss of tokens or money. The stack consists of up to 1024 32-byte words which can hold a maximum value of $2^{256}$. By adding a number to the max value, the new value rolls over to zero. Likewise for integer underflow, by subtracting from a zero value, the value rolls over to the maximum value~\cite{countercode}~\cite{conethbug} because EVM uses unsigned int256 types~\cite{howtobug}. Integer underflow vulnerabilities can allow an attacker to roll over his initial balance to the maximum value, thereby gaining access to a large token balance which he does not own. 

%Various libraries have been developed for high level programming languages for programming smart contracts such as solidity to mitigate these attacks. Bug detection tools have been developed to detect these vulnerabilities by using symbolic execution with SMT solvers~\cite{Oyente16}.




==> sections/acknowledgement.tex <==
This material is based upon work supported by NSF awards DMS-1737978, DGE-2039542, OAC-1828467, OAC-1931541, DGE-1906630, and ONR grant, N00014-20-1-2738.

==> sections/background.tex <==
% \begin{itemize}
% \color{blue}

In this section, we provide background information about the Ethereum virtual machine (EVM) and general types of vulnerabilities in smart contracts. After that, we introduce the metric learning and its motivations.


%\subsection{Smart Contracts}


\subsection{Ethereum Virtual Machine}

The Ethereum virtual machine (EVM) is one of the popular implementations of the smart contract framework. The EVM is a stack-based computer that takes input a sequence of bytecode instructions to complete a task. The EVM has a key-value persistent store, a memory, and a stack of 32-byte values. The EVM bytecode consists of opcodes and each opcode requires a particular set of fees to execute the instruction. The fee varies based on the function of the instruction. Figure \ref{fig:samplecounter} shows a sample EVM bytecode to perform addition and subtraction. In addition, fees are paid to persist data in the smart contract persistent store. Instructions will be executed only after the payment, ensuring that attackers cannot execute their malicious code without wasting their resources.

% Furthermore, Ethereum has two types of token standards which include ERC20 and ERC721. The ERC20 is a token standard that defines an interface to create custom cryptocurrencies while ERC721 is a standard that defines an interface for creating non-fungible assets used in representing unique objects on the Ethereum blockchain, such as was used for CryptoKitties. 

% \begin{figure}
% \centering
% \scalebox{1}{
% \includegraphics[width=\linewidth]{figures/contract_acct.pdf}
% }
% \caption{Ethereum smart contract account}
% \label{fig:conacct}
% \end{figure}

\lstdefinelanguage
   [x64]{Assembler}     % add a "x64" dialect of Assembler
   [x86masm]{Assembler} % based on the "x86masm" dialect
   % with these extra keywords:
   {morekeywords={PUSH1,JUMPI,MSTORE,MLOAD,CALLDATALOAD,JUMPDEST, ADD, %
                  POPFQ,PUSHFQ,SCASQ,STOSQ,IRETQ,RDTSCP,SWAPGS,PUSH,SUB,ADD, %
                  rax,rdx,rcx,rbx,rsi,rdi,rsp,rbp, %
                  r8,r8d,r8w,r8b,r9,r9d,r9w,r9b, %
                  r10,r10d,r10w,r10b,r11,r11d,r11w,r11b, %
                  r12,r12d,r12w,r12b,r13,r13d,r13w,r13b, %
                  r14,r14d,r14w,r14b,r15,r15d,r15w,r15b}} % etc.

\lstset{language=[x64]Assembler}
%, float,floatplacement=H
% \begin{lstlisting}[caption={Addition and subtraction program in EVM bytecode},captionpos=b,label={lst:samplecounter},basicstyle=\small,frame=single]
%  00000  PUSH1 0x01
%  00002  PUSH1 0x05
%  00004  SUB
%  00005  PUSH1 0x01
%  00007  PUSH1 0x05
%  00009  ADD
% \end{lstlisting}


\begin{figure}
    \centering
    \fbox{\begin{minipage}{20em}
    00000  PUSH1 0x01 \\
    00002  PUSH1 0x05 \\
    00004  SUB \\
    00005  PUSH1 0x01 \\
    00007  PUSH1 0x05 \\
    00009  ADD 
    \end{minipage}}
    \caption{Addition and subtraction program in EVM bytecode}
    \label{fig:samplecounter}
\end{figure}




\subsection{Common Ethereum Smart Contract Vulnerabilities }
%\input{sections/Vulnerability.tex}

\subsubsection{Reentrancy} 
Reentrancy is a well-known vulnerability with a recent TheDAO \cite{DAO} hack. In September of 2016, hackers stole over 3,600,000 Ether, or 60 million US Dollars, by exploiting a Reentrancy vulnerability in the contract code from the company TheDAO. 
The Reentrancy vulnerability comes from a function named \textit{fall-back} function. In Ethereum, when a contract calls another, the current execution will wait for the call to finish, leading to an issue where the callee can exploit the intermediate state of the caller.
% Since then, developers have changed codes to limit the function being accessed from malicious code. However, still a huge number of old contracts are vulnerable to the Reentrancy approach.

% The Reentrancy vulnerability starts from a function named \textit{fall-back} function. Every contract can only have one fall-back function. The fall-back function has no arguments and no return values. 
% This function will be called in two ways: First, when a contract receives a function call but no functions match; Second, when a contract receives Ethers. In Ethereum, when a contract calls another, the current execution waits for the call to finish. This can lead to an issue when the callee makes use of the intermediate state the caller is in. In other words, a malicious contract will write an external function call in its fall-back function. 

\subsubsection{Time Dependency}

Many applications on Ethereum require obtaining a block timestamp to decide what operations to do. Block timestamp is typically used in two situations: as a deterministic random seed and as a global timestamp in a distributed network, such as Castle\footnote{http://protect-the-castle.ether-contract.org/} and GovernMental\footnote{http://governmental.github.io/GovernMental/}. TheRun contract \cite{theRun} is an example of the former situation. TheRun contract uses the current timestamp to generate random numbers and award a jackpot based on the result.
The timestamp of the contract is dependent on the block timestamp, and block miners must agree on the block timestamp. Due to the synchronization, all contracts in the same block share the same timestamp. When a miner gets a new block, it can adjust the birth time of the new block, which could be 900 seconds in early Solidity versions. Although shortened to several seconds now, there is still a possibility of vulnerable timestamps.

\subsubsection{Mishandled Exceptions}
There are some ways for a contract to call another, including sending an instruction or calling a contract's function directly (\textit{e.g.,} ContractA.FunctionB()). 
Meanwhile, an exception can be raised in callee contracts because of insufficient gas, exceeding call stack limit, division by zero, array index out of bound,  \textit{etc}. If the exception happens, the callee contract will terminate, revert its state, and return false. A malicious caller contract can cause the send to fail deliberately, regardless of what the callee does to make a benefit. 

% 27.9\% of the contracts do not check the return values after calling other contracts via send \cite{luu2016making}. A malicious caller contract can cause the send to fail deliberately, regardless of what the callee does.
% Sometimes the attacker does not receive any direct benefit other than causing other users to lose their entitlement. But, in some other examples, the attacker can get  direct benefit (ex. GovernMental, this contract pays investors interest for their investments from the subsequent investments by others. An attacker can first invest his money. Then, he can cause failure in the previous investors, so he can receive his interest earlier! 

\subsubsection{Transaction-Ordering Dependence}

Since a transaction is in the memory pool for a short while, one can know what actions will occur before being included in a block. In the Ethereum Blockchain network, only miners can decide the order of transactions in a block. Therefore, the final state of a contract depends on the miner's decision about ordering the transactions. In this situation, the miners can conduct malicious behavior.

% for example, a smart contract offering a prize for providing the right solution to some problem. The contract owner can modify the prize as long as it has not been awarded, and users can submit their solutions to the problem to win the prize. On the other hand, the owner can track all submissions and manage the ordering of transactions. Let's consider the scenario when there is an unprocessed user transaction with a valid submission; the miner has the ability to check it out and then submit his own transaction thus reducing the value of the prize to zero. In such a case, the owner submission will be invoked first. And, the other user not only will not win the prize, but he has also submitted the solution for free! 


\subsubsection{Critical Instruction Vulnerabilities}

EVM bytecode consists of instructions that allow external smart contracts to call other smart contracts. These instructions include the CALL, CALLCODE, and DELEGATECALL instruction as shown in \autoref{fig:smartcall}. The CALL instruction allows a caller smart contract to call a target smart contract to modify the target contract's storage or variables. CALLCODE and DELEGATECALL enable a caller smart contract to reach a target smart contract and adjust the variable and storage in the caller's context. 
With these capabilities, attackers can inject code that can modify a smart contract's balance, change ownership or even self-destruct a smart contract and withdraw all the tokens in the contract.

% \subsubsection{Smart Contract Owner Hijack} 
% Each smart contract has an owner when deployed. For example, \cite{paritybug} show a code snippet for setting up a smart contract wallet for the Parity Ethereum Wallet from its GitHub repository. The \textit{initWallet} method is used to set the owner of the wallet. The \textit{initWallet} method should only be executed once in the lifetime of the smart contract. After initiating a smart contract, allowing changes to the ownership of a contract through a call to \textit{initWallet} can allow an arbitrary user to use methods such as delegate call to change the ownership of the contract. With the DELEGATECALL instruction, an attacker can pass a malicious payload to execute in the attacker's context. In this case, the attacker modified the owners of the smart contract by executing the \textit{initWallet} method. After changing the owner of the wallet contract, the attacker is able to kill the contract which results in all the funds in the wallet being withdrawn to the attacker.
% High-value attacks on the Parity Multisig smart contract \cite{paritybug, tether} were completed using this vulnerability to hijack the ownership of the smart contract.

\subsubsection{Arithmetic Vulnerabilities}
\label{arithvul}

Arithmetic vulnerabilities, \textit{a.k.a.} integer overflow and underflow, can occur during EVM code execution leading to loss of tokens or money. The stack consists of up to 1024 32-byte words, which can hold a maximum value of $2^{256}$. By adding a number to the max value, the new value rolls over to zero. Likewise for integer underflow, by subtracting from a zero value, the value rolls over to the maximum value \cite{conethbug}\footnote{https://github.com/CoinCulture/evm-tools/blob/master/analysis/guide.md} because EVM uses unsigned int256 types~\cite{howtobug}. 
Integer underflow vulnerabilities can allow an attacker to roll over his initial balance to the maximum value, thereby gaining access to a sizeable token credit which he does not own. Similar attacks can also happen by exploiting integer overflow.

%Various libraries have been developed for high level programming languages for programming smart contracts such as solidity to mitigate these attacks. Bug detection tools have been developed to detect these vulnerabilities by using symbolic execution with SMT solvers~\cite{Oyente16}.
\subsection{Metric Learning}

Classification algorithms in machine-learning-related tasks are well studied. Usually, classification is done by taking the outputs of the last fully connected (FC) layer of the network and feeding into the loss function, i.e., Cross-Entropy, during the learning process. While this process can usually achieve a good result, it ignores the quality of the features generated by the encoder because the loss function only focuses on the final results. Metric learning (or deep metric learning) takes a closer look at features generated by the encoder, especially the feature relation among classes. It tries to optimize such features with some loss functions. It makes the data points belonging to the same class closer and separates the data points belonging to different classes in the latent space.  The optimized representation features help facilitate classification tasks. Compared with general metric learning, i.e., triplet loss, pairwise contrastive learning conducts a more precise analysis and focuses on the hard samples. It assigns different weights to each pair and adjusts weights dynamically.

\begin{figure}
\centering
\scalebox{1}{
\includegraphics[width=1\linewidth]{figures/calldiag.pdf}
}
\caption{Smart contract CALL flow }
\label{fig:smartcall}
\end{figure}
% \end{itemize}

==> sections/biography.tex <==
\vspace{-10 mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/fengmi.png}}]{Feng Mi} is currently a Ph.D. student at the Big Data Analytics and Management Lab in the CS department, at the University of Texas at Dallas. He received an M.S. degree in Computer Engineering from University of Delaware in 2017. His main research interests lie in blockchain vulnerability detection, metric learning,  meta-learning, and cyber-security.
\end{IEEEbiography}
% \vspace{-18 mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/chenzhao.jpg}}]{Chen Zhao} is a Senior Research and Development Engineer at Kitware Inc. Prior to working at Kitware Inc, he received his Ph.D. in Computer Science from the University of Texas at Dallas in 2021. In 2016, he received dual M.S. degrees in computer science and biomedical science from University at Albany, SUNY and Albany Medical College, respectively. His researches focus on Machine Learning, Deep Learning, Data Mining, and Computer Vision.
\end{IEEEbiography}
% \vspace{-10 mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/zhuoyiwang.jpg}}]{Zhuoyi Wang} is currently a Ph.D student at the Big Data Analytics and Management Lab in the CS department, at the University of Texas at Dallas. His research interests focus on the area of stream mining, semi-supervised learning and cyber-security, especially the learning from limited labeled data in the non-stationary stream settings. His recent projects include resource constrained stream mining approach, and designing self-supervised learning models in the program embedding.
\end{IEEEbiography}
% \vspace{-15 mm}
\begin{IEEEbiography}[{\includegraphics[width=2.5in,height=1.25in,clip,keepaspectratio]{figures/sadaf.jpg}}]{Sadaf MD Halim} is a PhD student of Computer Science at The University of Texas at Dallas (UTD), with research interests spanning blockchains, federated learning, graph networks and medical informatics. Prior to this, he obtained a Master of Science (MSc) in Computer Science at UTD, and a Bachelor of Science (BSc) in Computer Science and Engineering at the Islamic University of Technology (IUT) in Dhaka, Bangladesh.
\end{IEEEbiography}
% \vspace{-15 mm}
\begin{IEEEbiography}[{\includegraphics[width=2.5in,height=1.25in,clip,keepaspectratio]{figures/xiaodi.JPG}}]{Xiaodi Li }  is currently a Ph.D. student at the Big Data Analytics and Management Lab in the CS department, at the University of Texas at Dallas. Her current research interests are Artificial Intelligence, Machine Learning, and Natural Language Processing. Her research covers continual learning and lifelong learning in NLP area especially in reducing the catastrophic forgetting during the learning process, and semi-supervised learning on imbalanced tabular security data
\end{IEEEbiography}
% \vspace{-15 mm}
% \vspace{-15 mm}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,height=1.1in,clip,keepaspectratio]{figures/zhouxiang.jpg}}]{Zhouxiang Wu} received the M.S. degrees in Computer Science from the University of Texas at Dallas in 2021, where he is currently pursuing the Ph.D. degree in computer science. His research interests include resource allocation, control system, reinforcement learning and federated learning.
\end{IEEEbiography}
% \vspace{-15 mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/LatifurKhan.jpg}}]{Latifur Khan} (Fellow, IEEE) is currently a full Professor (tenured) in the Computer Science department at the University of Texas at Dallas, USA where he has been teaching and conducting research since September 2000. He received his Ph.D. degree in Computer Science from the University of Southern California (USC) in August of 2000. He is an ACM Distinguished Scientist and a IEEE Fellow. He has received prestigious awards including the IEEE Technical Achievement Award for Intelligence and Security Informatics. Dr. Khan has published over 170 papers in 40 journals, in peer reviewed conference proceedings, and in three books. His research areas cover data mining, big data management, and analytics.
 
\end{IEEEbiography}
% \vspace{-15 mm}
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/hamlen.png}}]{Kevin W. Hamlen} received the BS degree in computer science and mathematics from Carnegie Mellon University, in 1998, and the MS and PhD degrees in computer science from Cornell University, in 2002 and 2006, respectively. He is an assistant professor with the Computer Science Department, University of Texas at Dallas. His research applies and extends compiler theory,
% functional and logic programming, and automated program analysis technologies toward the development of scientifically rigorous software security systems.
 
% \end{IEEEbiography}
% \vspace{-15 mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Thuraisingham.jpg}}]{Bhavani Thuraisingham} (Fellow, IEEE) is the Louis A. Beecherl, Jr. distinguished professor of Computer Science and the executive director of the Cyber Security Research and Education Institute (CSI) at The University of Texas at Dallas. She is an elected fellow of the AAAS, the British Computer Society, and the SPDS (Society for Design and Process Science). She is the reciepient of the IEEE CS 1997 Technical Achievement Award, the 2010 Research Leadership Award presented by IEEE ITS and IEEE SMC, and the 2010 ACM SIGSAC Outstanding Contributions Award.
 
\end{IEEEbiography}













==> sections/results.tex <==
The initial benchmark construction and feature extraction process were conducted on an Intel machine having Core-i7 3.40GHz CPU with 64 GB of RAM, running a standard Ubuntu Linux version 16.04 LTS. 
\textcolor{red}{We also set ...}


\begin{table}[t]
	\centering
	\begin{tabular}{|c|c|c|c|c|c| } \hline
		\textbf{Model}& \textbf{Accuracy}& \textbf{Precision} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUC score} \\ \hline
		KNN (k=3) & 0.59 & 0.65 & 0.60 & 0.62 & 0.2 \\ \hline
	    Random Forest  & 0.76 & 0.76 & 0.77 & 0.77 \\ \hline
	    SVM (Linear) &  0.72 &  0.73 &  0.73 &  0.73 \\ \hline
	    %LSTM & & & & \\ \hline
		BiLSTM & 0.87 & 0.80 & 87.1 & 0.83 \\ \hline
		BiLSTM with & & & & \\ 
		Attention & & & & \\ \hline
		
	\end{tabular}
	\caption{Comparison of the proposed method with KNN, Random Forest, and SVM}
	\label{Tab:result}
\end{table}

==> sections/temp.tex <==
% The increase in the adoption of decentralized cryptocurrency systems has resulted in the deployment of smart contracts to provide various services such as the emerging decentralized finance(DeFi) systems. 
Smart contracts are autonomous applications that execute on the blockchain in a decentralized way. With smart contracts, arbitrary computations can be performed in addition to transaction-based systems. Through the blockchain technique, different entities can interact without a centralized authority \cite{ruan2019fine, frey2019dietcoin}. 
%Common distributed consensus algorithm used to enforce the integrity of the distributed ledger includes proof-of-work, proof-of-stake, and proof-of-time~\cite{crosby2016blockchain, bitcoin, bitcoin}.
Smart contracts can be used all across the chain from financial services to healthcare to insurance \cite{griggs2018healthcare,cohn2017smart,buterin2014next}. Due to the rapid growth in their deployments, various vulnerabilities have been exploited by attackers to steal cryptocurrencies worth millions of dollars \cite{hynes2018demonstration}. \textcolor{red}{So the requirement of vulnerability detection has attract more and more attention in recent times. }

Smart contracts are commonly written in a high-level language, such as Ethereum's Solidity, then it is translated to low-level bytecode for deployment on the blockchain. A blockchain can be seen as a public virtual machine where the bytecode of the smart contracts is easy to get. Using the Application Binary Interface (ABI), users can interact with a deployed smart contract to complete tasks. The challenge to detect the vulnerabilities is
that most smart contracts’ solidity code is not provided and
people can only get the bytecode of these smart contracts.
This indicates developing tools to detect vulnerabilities using
bytecode is more practical for users.

Currently, Ethereum \cite{buterin2014next} and Cardano~\cite{cardano} are two types of blockchains with smart contract capabilities. Ethereum has become the \textit{de facto} standard platform for smart contract development, with a market capitalization of \$46B (USD)\footnote{https://coinmarketcap.com/currencies/ethereum/} and having \$6.5B (USD)\footnote{https://defipulse.com/} cryptocurrencies locked in its smart contracts in the middle of 2020. Due to this reason, we focus particularly on Ethereum smart contracts in this study.



%As a result of these attacks, best practices that govern the development of smart contract applications have been proposed to mitigate such attacks. Implementing these best practices have been challenging and cumbersome due to the number of programming languages available to write smart contracts applications. These languages include Solidity \cite{solidity}, which has similar syntax to Javascript, Haskell \cite{haskell}, Vyper \cite{vyper} and, Isabelle/HOLs \cite{hol}. However, convincing developers to learn new languages is challenging and gaining the proficiency to develop correct and secure code in a new language can be demanding.
%By leveraging the Ethereum framework, we proposed and developed an Ethereum bytecode rewriting framework that rewrites raw bytecode and apply code protection and safety policies. In addition, we implemented a bytecode verification system to ensure the modified code is equivalent in outcome as the original code. We evaluated our system using both integer overflow[ARITH1] and integer underflow[ARITH2] code protection policies. Furthermore, we evaluated the performance of our system by measuring the file size and instruction count overhead.

Previous works in smart contract defense focused on discovering vulnerabilities in smart contracts. Oyente\cite{Oyente16}, Osiris \cite{osir}, TeEther\cite{tether} and Zeus\cite{zeus} performed vulnerability discoveries by leveraging symbolic execution, Z3 solvers \cite{de2008z3} and source code analysis by pre-defined rules. Symbolic execution has a scalability problem because of the time consuming in the execution procedure. On the other hand, rule-based systems rely on human experts to define different rules to detect bugs in the programs. There are also some works \cite{J2019fuzz,wang2020xg} which use basic machine learning models and a limited number of source codes as the dataset. 

We propose a framework  VSCL to address aforementioned issues. In VSCL, we select to use bytecodes as datasets.  Bytecodes can be easily acquired and have a large amount. So the detection made by the VSCL is more convincing and it is more practical compared to the tools used on limited source code. To better  reflect the program execution semantics, after converting the bytecodes to sequence of  operation codes by disassembler, we extract the control flow graph(CFG)  and adopt  depth first search method to form a new sequence of operations. After the Ngram and TFIDF processing, we use the formed feature matrix to feed in our developed  deep  neural  network  with  metric  learning loss  which encourages the same class closer to each other and separates the distance of different classes in the embedding space. It makes classification precisely by conducting similarity analysis and weight strategy at pairwise level.

Compared with all these works, the VSCL has the following characteristics: (1). VSCL does not rely on defined rules. It has its own view and it can auto extract and learn features. So  there is no need to update the rules regularly and has no worries in uncovering rules. (2). VSCL is a static approach meaning it does not need to execute the programs multiple times. When a smart contract comes, we only need to construct its feature vector and feed into the detection model.  (3). VSCL trains and makes detection using data which can be easily  acquired and has a large amount. So the detection made by the VSCL is more convincing and it is more practical. (4). VSCL does not adopt existing traditional machine learning models and we developed DNN with metric learning loss for making smart contract vulnerability detection specifically. 

In summary, the contributions of the proposed approach are as follows: 

%One downside of these methods is that many traditional NLP systems are utilized to extract high-level features, such as part of speech tags, shortest dependency path and named entities, which consequently results in the increase  of computational cost and additional propagation errors. Another downside is that designing features manually is time-consuming, and performing poor on generalization due to the low coverage of different training datasets.

\begin{itemize}

    \item In the feature engineering pipeline, we first convert the bytecode to a sequence of more readable low-level opcodes and construct its control flow graph(CFG). By traversing through CFG using depth first search, we get opcodes sequence which reflects the execution scenario. 
    
    \item We developed the metric learning-based  deep neural network, which encourages the same class closer to each other and separates the distance of different classes in the embedding space. It makes classification precisely by conducting similarity analysis and weight strategy at pairwise level.
 
    
	\item We empirically evaluate the proposed framework over real-world large-scaled Ethereum smart contract benchmark and compare its performance against other available machine learning-based approaches. The results show that our approach outperforms the other approaches. 
    
\end{itemize}

% In this study, we proposed a static framework VSCL that does not need to run the smart contract frequently and use large amounts of bytecode as a dataset. It is also based on a deep learning model, of which the auto-learned features are not pre-defined by human experts.
% %Previous works on program verification includes compiler certification \cite{Leroy:2009,evmverify,kframework}.  
% %Our work differs from these previous approaches in the following ways. 

% The key contributions of this study are as follows: 

% %One downside of these methods is that many traditional NLP systems are utilized to extract high-level features, such as part of speech tags, shortest dependency path and named entities, which consequently results in the increase  of computational cost and additional propagation errors. Another downside is that designing features manually is time-consuming, and performing poor on generalization due to the low coverage of different training datasets.

% \begin{itemize}

%     \item Since the high-level source code of smart contracts are usually not provided, here we only need bytecode as an input in VSCL framework. In our feature engineering pipeline, we convert the bytecode to a sequence of more readable low-level opcodes and construct its control flow graph. Then, we traverse these graphs to transform them into vectors which reflect the semantics of the code.
    
%     \item We use deep learning for vulnerability detection in Ethereum smart contracts. This approach has great potential because deep learning does not need human experts to manually define features and rules, meaning that vulnerability detection can be automated. We developed  metric learning-based  deep neural network which encourage the same class closer to each other and separate the distance of different classes in the embedding space by doing pairwise analysis. 
    
% 	\item We empirically evaluate the proposed framework over real-world large-scaled Ethereum smart contract benchmark and compare its performance against other available machine learning-based approaches. The results show that our approach outperforms the other approaches. 
    
% \end{itemize}

%The contribution of this paper is using BLSTM with attention mechanism, which can automatically focus on the words that have decisive effect on classification, to capture the most important semantic information in a sentence, without using extra knowledge


%We are currently working to detect vulnerabilities in smart contracts. In this study, we will disassemble the low-level Ethereum Virtual Machine (EVM) bytecode, and then convert it to control flow graph (CFG). Here, CFG is a labeled directed graph that is defined as G = (V, E, α) where V is the set of vertices, E ⊆ V × V is the set of directed edges, α is the vertex labels. Given a set of training examples T = {(xi, yi)} where xi ∈ X is a graph, and yi ∈ Y = {+ 1, − 1} is a target label, the graph classification problem is to induce the mapping f: X → Y. After CFG extraction, we need to convert it to a feature matrix by using node2vec [Node2vec], GraphSAGE [GraphSage], etc. Then, we apply our novel online metric learning framework to detect vulnerable smart contracts in stream on data. Good quality similarity metrics can significantly facilitate the performance of many large-scale, real-world applications. 
%In this approach, we present a new online metric learning framework that attempts to tackle the challenge by learning a ANN-based metric with adaptive model complexity from a stream of constraints. We provide detailed discussion in section B.6 [WWWYang][WWWyifan].


% This paper is organized as follows: 
% In Section \ref{sec:smart_background}, we discuss the Ethereum virtual machine and present the well-known vulnerabilities in Ethereum smart contracts.
% In Section \ref{sec:smart_arc}, we introduce the stages of the vulnerability detection in smart contract pipeline.
% In Section \ref{sec:smart_evaluation}, we point out the benchmark and discuss results from our empirical analysis experiments.
% Related work is surveyed in Section \ref{sec:smart_related}. 
% Then, we will discuss our work limitations and future works in Section \ref{sec:smart_discussion}. 
% Finally, in Section \ref{sec:smart_conclusion}, we draw our conclusions.

